Panorama: A Framework to Support Collaborative Context Monitoring on Co-Located Mobile Devices

A key challenge in wide adoption of sophisticated context-aware applications is the requirement of continuous sensing and context computing. This paper presents Panorama, a middleware that identifies collaboration opportunities to offload context computing tasks to nearby mobile devices as well as cloudlets/cloud. At the heart of Panorama is a multi-objective optimizer that takes into account different constraints such as access cost, computation capability, access latency, energy consumption and data privacy, and efficiently computes a collaboration plan optimized simultaneously for different objectives such as minimizing cost, energy and/or execution time. Panorama provides support for discovering nearby devices and cloudlets/cloud, computing an optimal collaboration plan, distributing computation to participating devices, and getting the results back. The paper provides an extensive evaluation of Panorama via two representative context monitoring applications over a set of Android devices and a cloudlet/cloud under different constraints.

==> infrastructure.tex <==
\subsection{Impact of Collaboration Opportunities}
%\subsection{Impact of Collaborating Opportunities on Collaboration Decisions}
\label{sec:infrastructure}

\begin{figure}
\centering
\includegraphics[scale=0.7]{WhenToOffload.pdf}
\caption{Benefits from various collaboration opportunities}
\label{fig:whenl}
\end{figure}

%As mentioned in Section ``Introduction'', a user is typically in the vicinity
%of several other mobile devices and perhaps cloud/cloudlet.
Different
offloading opportunities provide different performance and energy
benefits as well as incur additional communication and computation overheads.
A key question for a user is when to offload and how.
%Panorama utilizes this information along with the initiator's performance
% objectives to ensure effective and beneficial collaborations.
To answer this question, we first 
investigate how different opportunities from various
combinations of collaboration impact the efficacy of the devised plans in
the context of speech recognition. The results here apply to the tasks that
are similar in nature to speech recognition (i.e., compute-intensive and
can exploit parallelism). Figure~\ref{fig:when} shows the results of an
experiment where we use Panorama to devise collaboration plans that achieve
maximum gain in terms of energy and time combined by assigning equal weight
to those two objectives. The gain is measured by comparing the
improvement from the collaboration plan to the local execution on the
initiating node. Note that the results here also consider the overhead of Bluetooth and Wi-Fi (time and energy), which we measured manually. For Bluetooth, the measured rate and consumed power during file
transmission is 2.1 Mb/s and 440mW respectively. Bluetooth v.3 + HS sends
data at a much higher rate of 24  Mb/s, but Android APIs still don't provide
support for it. As for Wi-Fi, we report an average of around 1 MB/s to
send files to the cloud with a consumption rate of 1500mW. These measurements
are consistent with those reported in
\cite{friedman2013power}. Also, notice  that Panorama can be easily extended
to use network profiling similar to \cite{cuervo2010maui} to account
for online network characteristics. 

We consider three diferent cases. In the first scenario, a high-end
mobile device (a smartphone with quad-core processor) is engaged in a
collaboration with two lower-end smartphones to process a 4 MB speech
recognition task. The achieved combined gain is $19.27\%$, with a breakdown
of $47\%$ gain in time and $8.56\%$ loss in energy. We see that while an
overall gain can be achieved from exploiting parallelism, engaging lower-end
nodes in collaboration leads to more energy consumption 
%including the Bluetooth energy overhead caused offloaded portions of the file to be processed with slower speeds (though in parallel), which contributed jointly with the Bluetooth energy overhead to cause more energy consumption 
than in the case of local execution. In contrast, in the second case where
the initiator is a low-end smartphone and the high-end device is one of
the collaborators, collaboration leads to gain %This in turn caused the offloaded portion to be processed more efficiently 
in both time and energy when compared to local execution, achieving a
combined gain of $54.98\%$. We also consider a scenario of offloading the
task to a cloud server (an Amazon EC2 server used as a speech recognition
server), which achieves a large combined gain of $81.58\%$ by shipping
speech recognition, a compute-intensive task to a cloud server. The results
of this experiment demonstrate that Panorama is quite effective in 
identifying when and how to offload computation task to the various
collaborators to realize the initiator's performance/energy objectives.

